Code Transformation Rule Synthesis using LLMs: Potential and Limits

Due to their black-box nature, LLMs suffer from limited explain- ability and a lack of determinism. Their usage cost can also rise, particularly with repetitive tasks on large codebases. To mitigate this, we conduct a novel empirical study targeting three domain- specific languages for transformation rules, namely Comby, GritQL, and Ast-Grep. We evaluate three LLMs (GPT-5.4, GPT-oss-120B, and Llama3.1-8B) on six diverse datasets covering four software- evolution tasks: API misuse correction, program repair, API migra- tion, and language version migration. Our results provide evidence that transformation rule synthesis moves beyond proof-of-concept with strong frontier models. GPT-5.4 achieves consistently high rule applicability rates and produces transformations closest to the ground truth across most benchmarks. Smaller and open-weight GPT-oss-120B and Llama3.1-8B models remain effective for simpler, localized changes but struggle with complex migration scenarios. We also observe non-negligible generalizability through the usage of meta-variables and through a high reuse score in the first quartile of many datasets. Finally, when compared to the anti-unification algorithm, LLMs outperform it in correctness, but underperform in rule applicability. Overall, our results show great potential for LLMs to generate sound, correct, generalizable, and reusable rules.

==> authors.tex <==
\title[Code Transformation Rule Synthesis using LLMs: Potential and Limits]{Code Transformation Rule Synthesis using LLMs:\newline Potential and Limits}

\author{Axel Allain}
\correspondingauthor
\orcid{0009-0009-9088-6178}
\affiliation{
  \institution{Univ Rennes, INRIA, CNRS, IRISA}
  \city{Rennes}
  \country{France}
}
\email{axel.allain@inria.fr}

\author{Aymeric Blot}
\orcid{0000-0003-0485-5279}
\affiliation{
  \institution{Univ Rennes, INRIA, CNRS, IRISA}
  \city{Rennes}
  \country{France}
}
\email{aymeric.blot@irisa.fr}

\author{Djamel Eddine Khelladi}
\orcid{0000-0002-2218-650X}
\affiliation{
  \institution{Univ Rennes, INRIA, CNRS, IRISA}
  \city{Rennes}
  \country{France}
}
\email{djamel-eddine.khelladi@irisa.fr}

\author{Mathieu Acher}
\orcid{0000-0003-1483-3858}
\affiliation{
  \institution{Univ Rennes, INRIA, CNRS, IRISA}
  \city{Rennes}
  \country{France}
}
\email{mathieu.acher@irisa.fr}

==> figures/distribution.tex <==
\begin{figure*}[t]
\centering

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={Galappaththi et al.},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,67.5) (x1,81.8) (x2,24.0) (x3,53.5) (x4,80.0) (x5,0.0) (x6,53.8) (x7,67.5) (x8,17.6) (x9,58.5) (x10,46.5) (x11,23.8) };
\addplot coordinates { (x0,62.8) (x1,20.9) (x2,14.0) (x3,53.5) (x4,37.2) (x5,0.0) (x6,32.6) (x7,62.8) (x8,7.1) (x9,55.8) (x10,46.5) (x11,23.3) };
\addplot coordinates { (x0,67.5) (x1,81.8) (x2,24.0) (x3,53.5) (x4,80.0) (x5,0.0) (x6,53.8) (x7,67.5) (x8,17.6) (x9,58.5) (x10,46.5) (x11,23.8) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={ManySStuBs4J},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,69.2) (x1,0.0) (x2,29.5) (x3,68.2) (x4,72.7) (x5,0.0) (x6,71.5) (x7,82.0) (x8,21.4) (x9,68.5) (x10,76.1) (x11,40.6) };
\addplot coordinates { (x0,68.0) (x1,0.0) (x2,10.8) (x3,66.7) (x4,60.6) (x5,0.0) (x6,41.9) (x7,70.1) (x8,2.8) (x9,67.8) (x10,75.4) (x11,40.3) };
\addplot coordinates { (x0,68.8) (x1,0.0) (x2,29.5) (x3,68.1) (x4,72.6) (x5,0.0) (x6,71.3) (x7,81.9) (x8,20.8) (x9,68.2) (x10,75.8) (x11,40.4) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={Defects4J},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,33.2) (x1,0.0) (x2,10.5) (x3,32.3) (x4,37.7) (x5,0.0) (x6,46.6) (x7,56.0) (x8,0.0) (x9,11.7) (x10,37.8) (x11,12.9) };
\addplot coordinates { (x0,30.5) (x1,0.0) (x2,4.0) (x3,30.5) (x4,29.8) (x5,0.0) (x6,24.4) (x7,43.9) (x8,0.0) (x9,11.5) (x10,37.8) (x11,12.9) };
\addplot coordinates { (x0,33.1) (x1,0.0) (x2,10.5) (x3,32.2) (x4,37.7) (x5,0.0) (x6,45.4) (x7,56.0) (x8,0.0) (x9,11.7) (x10,37.8) (x11,12.9) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={BugsInPy},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,22.4) (x1,33.3) (x2,6.9) (x3,19.0) (x4,28.9) (x5,0.0) (x6,31.5) (x7,54.1) (x8,5.8) (x9,18.0) (x10,33.5) (x11,9.9) };
\addplot coordinates { (x0,20.9) (x1,5.4) (x2,1.6) (x3,18.4) (x4,19.7) (x5,0.0) (x6,14.3) (x7,44.7) (x8,1.6) (x9,17.9) (x10,33.5) (x11,9.8) };
\addplot coordinates { (x0,22.4) (x1,33.3) (x2,6.9) (x3,19.0) (x4,28.9) (x5,0.0) (x6,31.5) (x7,54.1) (x8,5.8) (x9,18.0) (x10,33.5) (x11,9.9) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={PyMigBench},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,43.2) (x1,89.9) (x2,12.2) (x3,41.7) (x4,63.5) (x5,0.0) (x6,46.1) (x7,57.5) (x8,8.4) (x9,35.2) (x10,40.0) (x11,17.3) };
\addplot coordinates { (x0,39.3) (x1,31.1) (x2,4.8) (x3,39.0) (x4,35.9) (x5,0.0) (x6,22.5) (x7,46.8) (x8,2.0) (x9,35.0) (x10,40.0) (x11,17.2) };
\addplot coordinates { (x0,43.2) (x1,89.9) (x2,12.2) (x3,41.7) (x4,63.5) (x5,0.0) (x6,46.1) (x7,57.5) (x8,8.4) (x9,35.2) (x10,40.0) (x11,17.3) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=7.2cm,
    ybar,
    bar width=3pt,
    ymin=0, ymax=100,
    ylabel={Rate (\%)},
    title={JMigBench},
    symbolic x coords={x0,x1,x2,x3,x4,x5,x6,x7,x8,x9,x10,x11},
    xtick=data,
    xticklabels={{Comby (RAG)\\GPT-oss-120B},{Comby (RAG)\\GPT5.2},{Comby (RAG)\\Llama3.1-8B},{Comby (no RAG)\\GPT-oss-120B},{Comby (no RAG)\\GPT5.2},{Comby (no RAG)\\Llama3.1-8B},{Ast-Grep\\GPT-oss-120B},{Ast-Grep\\GPT5.2},{Ast-Grep\\Llama3.1-8B},{GritQL\\GPT-oss-120B},{GritQL\\GPT5.2},{GritQL\\Llama3.1-8B}},
    xticklabel style={rotate=60, anchor=east, align=right, font=\scriptsize},
    ymajorgrids=true,
    grid style={dashed, gray!30},
    legend style={font=\scriptsize, at={(0.5,1.18)}, anchor=south, legend columns=3},
    enlarge x limits=0.02,
]
\addplot coordinates { (x0,68.9) (x1,88.2) (x2,28.0) (x3,64.4) (x4,80.0) (x5,0.0) (x6,30.8) (x7,57.6) (x8,0.0) (x9,22.2) (x10,26.7) (x11,6.8) };
\addplot coordinates { (x0,68.9) (x1,33.3) (x2,15.6) (x3,64.4) (x4,62.2) (x5,0.0) (x6,17.8) (x7,42.2) (x8,0.0) (x9,22.2) (x10,26.7) (x11,6.7) };
\addplot coordinates { (x0,68.9) (x1,88.2) (x2,28.0) (x3,64.4) (x4,80.0) (x5,0.0) (x6,30.8) (x7,57.6) (x8,0.0) (x9,22.2) (x10,26.7) (x11,6.7) };
\legend{AST / Success, AST / All, AST / AR}
\end{axis}
\end{tikzpicture}

\vspace{0.6cm}
\caption{AST-match distribution across datasets, tools, and models. AST / Success = ast\_match\_rate, AST / All = ast\_match\_all\_rate, AST / AR = ast\_match\_given\_AR.}
\label{fig:ast-match-distribution}
\end{figure*}

==> figures/rule_reuse_many.tex <==
\begin{figure}[t]
\centering
\ifBlueHighlights
\includegraphics[width=\linewidth]{figures/rule_reuse_manysstubs4j_blue.pdf}
\else
\includegraphics[width=\linewidth]{figures/rule_reuse_manysstubs4j.pdf}
\fi
\caption{\camera{Number of matches per rule obtained with GPT-oss-120B, GPT-5.4, and Llama 3.1-8B on ManySStuBs4J.}}
\label{fig:reuse_score_many}
\end{figure}

==> recommendations-old.tex <==
\section{Discussion and Recommendations}
\textbf{Discussion}

Our results highlight important limitations related to dataset characteristics. In particular, datasets such as Defects4J, BugsInPy, and PyMigBench appear significantly more challenging due to the size and complexity of their diffs. These transformations are often not well-suited for DSL-based rule generation, as they involve large, heterogeneous modifications that do not consistently share common structures between the “before” and “after” code. As a consequence, the use of metavariables becomes more difficult, limiting the ability of models to infer concise and reusable transformation rules. These findings suggest that current benchmarks are not always aligned with the assumptions underlying transformation rule generation.

More generally, our results show that models perform substantially better on simple, localized transformations, such as one-line code changes (RQ4). In contrast, large and complex diffs are harder to generalize into a single transformation rule. While GPT-5.4 demonstrates a stronger ability to handle such cases, this capability appears to rely on implicitly decomposing complex transformations into smaller, more manageable subrules. This is particularly important given that transformation languages such as GritQL and Ast-grep rely on AST node matching, which makes large rigid rules difficult to apply effectively. Conversely, GPT-oss-120B tends to avoid generating large transformation rules and instead produces smaller, fragmented rules, which reduces overall performance. These observations suggest that explicitly encouraging decomposition through prompt engineering could further improve the effectiveness of advanced models.

We also observe notable differences across model families. Llama-based models achieve lower overall performance, largely due to limitations in context window size, timeout constraints, and weaker reasoning capabilities. However, they remain effective at generating simple, one-line transformation rules. This makes them particularly suitable for local deployment scenarios, where privacy constraints are critical and lightweight models are preferred, even at the cost of reduced expressiveness.

In addition, we identify recurring failure modes in rule generation. Models may overgeneralize transformation rules, leading to excessive and potentially incorrect matches, or undergeneralize them, resulting in overly specific rules that fail to transfer to new contexts. This highlights the difficulty of balancing precision and generality when inferring transformation rules, and suggests the need for mechanisms to better control rule scope.

These findings also reveal an inherent trade-off between model capability, operational cost, and data privacy. More powerful models are better able to handle complex transformations but often require external APIs and higher computational resources, raising cost and confidentiality concerns. In contrast, smaller local models provide stronger privacy guarantees and lower costs, but are limited to simpler transformations. This trade-off suggests that hybrid approaches, combining different models depending on task complexity, may be a promising direction.

Finally, our experiments show that retrieval-augmented generation (RAG) can negatively impact performance in this context. The retrieved examples exhibit a strong bias toward Python transformations \red{[ok say this above in the RQs, i feel you did not]}, introducing domain bias when applied to other contexts. Moreover, the limited number of retrieved examples (eight in our setup) leads to sampling bias, where some examples are more relevant than others. This can misguide the model and increase the likelihood of hallucinated or inappropriate transformation rules. These results emphasize the importance of retrieval quality and diversity when applying RAG to transformation rule generation.

\textbf{Recommendations}
    
Our results suggest several recommendations for different stakeholders.

\textbf{For Developers.}
Transformation rule generation can be effectively leveraged to automate repetitive code modifications from minimal input. In particular, developers can generate a rule from a single example and apply it recursively across a codebase, significantly reducing manual effort. However, our findings indicate that complex refactorings are better handled when decomposed into smaller, composable subrules. This modular approach improves both reliability and interpretability of the generated transformations. Furthermore, these findings suggest that transformation rule generation is best suited for integration into semi-automated workflows rather than fully autonomous refactoring systems. For instance, such techniques could be embedded into IDEs, where developers provide a representative code diff and receive suggested transformation rules that can be interactively reviewed and applied across the codebase. Additionally, an alternative usage scenario consists in generating transformation rules from an input code and a natural language query, enabling developers to describe the intended modification while leveraging LLMs to synthesize the corresponding rule.

\textbf{For Researchers.}
Rule generation provides a powerful abstraction for analyzing software evolution at scale. Automatically inferred rules can be used to extract recurring transformation patterns from large datasets, enabling systematic studies of code changes. In particular, researchers can leverage these rules to analyze the distribution and frequency of common bug patterns, API misuses, and migration practices across projects.
Furthermore, transformation rules offer a structured and interpretable representation of LLM outputs, which can facilitate their analysis and evaluation. They can also be integrated into fuzzing pipelines, where generated rules are used to systematically explore variations of code transformations. Finally, rule mining can support dataset augmentation and the mining of software repositories, enabling richer and more diverse benchmarks.

\textbf{Across Stakeholders.}
Transformation rules generation also raises important practical considerations regarding deployment contexts. In settings involving sensitive or proprietary code bases, local models provide a viable solution for generating transformation rules while preserving data privacy. Although such models may be limited to lower-complexity transformations, they remain effective for a wide range of routine maintenance tasks. Thus, rule generation techniques can be integrated into existing workflows across diverse environments without requiring exposure of confidential data.

==> tables/tab-results-rq1-datasets-agg.tex <==
\begin{table}[H]
\centering
\caption{Soundness of Generated Transformation Rules per Scenario and LLM (RA\%) \red{Stdev error}}
\label{tab:results-rq1-datasets-agg}
\begin{tabular}{l c c c}
\toprule
\textbf{Scenarios}
& \textbf{GPT-oss-120B}
& \textbf{GPT5.4}
& \textbf{Llama3.1-8B} \\
\cmidrule(lr){2-4}
& \textbf{RA\%} & \textbf{RA\%} & \textbf{RA\%} \\

\multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
Mean over DSLs & 87.2 $\pm$ 15.6 & 97.1 $\pm$ 3.0 & 69.4 $\pm$ 21.8 \\
\midrule
\multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
Mean over DSLs & 85.8 $\pm$ 19.5 & 89.1 $\pm$ 10.4 & 55.3 $\pm$ 34.3 \\
\midrule
\multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
Mean over DSLs & 83.2 $\pm$ 20.1 & 89.0 $\pm$ 7.0 & 57.8 $\pm$ 29.0 \\
\midrule
\multicolumn{4}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
Mean over DSLs & 89.4 $\pm$ 18.3 & 92.8 $\pm$ 11.3 & 67.8 $\pm$ 27.6 \\

\bottomrule
\end{tabular}
\caption{\textit{Metric: RA = Rule Applicability rate}}
\end{table}

==> tables/tab-results-rq1-datasets.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{4pt}
\footnotesize
\caption{Soundness of Generated Transformation Rules per Scenario, Tool, and LLM (RA\%)}
\label{tab:results-rq1-datasets}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l l c c c @{}}
\toprule
\textbf{Scenario} & \textbf{Tool}
& \textbf{GPT-oss-120B}
& \textbf{GPT5.4}
& \textbf{Llama3.1-8B} \\
\cmidrule(lr){3-5}
& & \textbf{RA\%} & \textbf{RA\%} & \textbf{RA\%} \\

\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
& Comby & 93.0 & 95.3 & 58.1 \\
& Comby (no RAG) & 100.0 & 100.0 & 81.4 \\
& Ast-Grep & 60.5 & 93.0 & 40.5 \\
& GritQL & 95.3 & 100.0 & 97.7 \\
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
& Comby & 94.9 & 97.4 & 32.6 \\
& Comby (no RAG) & 96.5 & 76.9 & 74.4 \\
& Ast-Grep & 52.6 & 82.2 & 14.4 \\
& GritQL & 99.2 & 99.8 & 99.9 \\
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
& Comby & 91.1 & 89.6 & 39.3 \\
& Comby (no RAG) & 93.6 & 85.3 & 68.6 \\
& Ast-Grep & 48.8 & 81.3 & 23.6 \\
& GritQL & 99.5 & 100.0 & 99.5 \\
\multicolumn{5}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
& Comby & 100.0 & 100.0 & 55.6 \\
& Comby (no RAG) & 100.0 & 97.8 & 86.7 \\
& Ast-Grep & 57.8 & 73.3 & 28.9 \\
& GritQL & 100.0 & 100.0 & 100.0 \\


\bottomrule
\end{tabular*}
\caption*{\textit{Metrics: RA = Rule Applicability rate}}
\end{table}

==> tables/tab-results-rq1-dsl.tex <==
\begin{table}[H]
\centering
\caption{Soundness of Generated Transformation Rules per Tool and LLM (RA\%)}
\label{tab:results-rq1-dsl}
\begin{tabular}{l c c c}
\toprule
\textbf{Tool}
& \textbf{GPT-oss-120B}
& \textbf{GPT5.4}
& \textbf{Llama3.1-8B} \\
\cmidrule(lr){2-4}
& \textbf{RA\%} & \textbf{RA\%} & \textbf{RA\%} \\

Comby & 94.8 & 96.2 & 41.8 \\
Comby (no RAG) & 97.2 & 85.6 & 64.0 \\
Ast-Grep & 54.2 & 82.4 & 22.4 \\
GritQL & 98.8 & 99.9 & 99.5 \\

\bottomrule
\end{tabular}
\caption{\textit{Metric: RA = Rule Applicability rate}}
\end{table}

==> tables/tab-results-rq1-tools.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{4pt}
\footnotesize
\caption{Soundness of Generated Transformation Rules per Dataset and LLM (Grouped by Scenario)}
\label{tab:results-rq1-tools}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l c c c @{}}
\toprule
\textbf{Benchmarks}
& \textbf{GPT-oss-120B}
& \textbf{GPT5.4}
& \textbf{Llama3.1-8B} \\
\cmidrule(lr){2-4}
& \textbf{RA\%} & \textbf{RA\%} & \textbf{RA\%} \\
\midrule

\multicolumn{4}{l}{
\begin{tabular}[c]{@{}l@{}}
\textbf{API Misuse} \end{tabular}
} \\
\midrule
\begin{tabular}[c]{@{}l@{}} Galappaththi et al. \\ \footnotesize (n=43)\end{tabular} 
& 87.2 & 97.1 & 69.4 \\

\midrule
\multicolumn{4}{l}{
\begin{tabular}[c]{@{}l@{}}
\textbf{Program Repair} \end{tabular}
} \\
\midrule
\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528)\end{tabular} 
& 88.7 & 92.0 & 37.5 \\
\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427)\end{tabular} 
& 84.9 & 89.1 & 52.3 \\
\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=559)\end{tabular} 
& 83.9 & 86.2 & 56.7 \\

\midrule
\multicolumn{4}{l}{
\begin{tabular}[c]{@{}l@{}}
\textbf{API Migration} \end{tabular}
} \\
\midrule
\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=605)\end{tabular} 
& 83.2 & 89.0 & 57.8 \\

\midrule
\multicolumn{4}{l}{
\begin{tabular}[c]{@{}l@{}}
\textbf{Language Version Migration}\end{tabular}
} \\
\midrule
\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45)\end{tabular} 
& 89.4 & 92.8 & 67.8 \\

\bottomrule
\end{tabular*}
\caption*{\textit{Metric: RA = Rule Applicability rate}}
\end{table}

==> tables/tab-results-rq1.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.5pt}
\footnotesize
\caption{Soundness of Generated Transformation Rules per Dataset, Tool, and LLM (Grouped by Scenario)}
\label{tab:results-rq1}
\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l l *{3}{c c c} @{}}
\toprule
\textbf{Benchmarks} & \textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
& & \textbf{F} & \textbf{RA\%} & \textbf{NT}
  & \textbf{F} & \textbf{RA\%} & \textbf{NT}
  & \textbf{F} & \textbf{RA\%} & \textbf{NT} \\
\midrule

\multicolumn{11}{l}{\textbf{API Misuse}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Galappaththi et al. \\ \footnotesize (n=43)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 3 & 93.0 & 192 & \textbf{2} & \textbf{95.3} & 208 & 18 & 58.1 & \textbf{166} \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{0} & \textbf{100.0} & \textbf{185} & \textbf{0} & \textbf{100.0} & 202 & 8 & 81.4 & 264 \\

& Ast-Grep & 17 & 60.5 & \textbf{170} & \textbf{3} & \textbf{93.0} & 228 & 25 & 40.5 & 342 \\

& GritQL & 2 & 95.3 & 253 & \textbf{0} & \textbf{100.0} & \textbf{215} & 1 & 97.7 & 293 \\
\midrule
\multicolumn{11}{l}{\textbf{Program Repair}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 9 & 98.9 & \textbf{90} & \textbf{5} & \textbf{99.2} & 225 & 335 & 36.6 & 212 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{12} & \textbf{97.9} & \textbf{88} & 88 & 83.5 & 171 & 128 & 76.1 & 995 \\

& Ast-Grep & 219 & 58.7 & 108 & \textbf{77} & \textbf{85.6} & \textbf{108} & 448 & 15.5 & 557 \\

& GritQL & 5 & 99.4 & \textbf{148} & 5 & 99.4 & 221 & \textbf{4} & \textbf{99.8} & 242 \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 34 & 92.3 & 160 & \textbf{4} & \textbf{99.1} & 211 & 264 & 38.0 & \textbf{124} \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{24} & \textbf{94.8} & \textbf{134} & 89 & 79.1 & 173 & 125 & 71.1 & 239 \\

& Ast-Grep & 203 & 53.8 & 152 & \textbf{92} & \textbf{78.4} & 179 & 426 & 0.0 & \textbf{0} \\

& GritQL & 6 & 98.6 & 201 & \textbf{0} & \textbf{100.0} & 240 & \textbf{0} & \textbf{100.0} & \textbf{174} \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=559)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 36 & 93.6 & \textbf{158} & \textbf{34} & \textbf{93.9} & 213 & 429 & 23.3 & 159 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{18} & \textbf{96.8} & \textbf{149} & 178 & 68.2 & 169 & 134 & 76.0 & 201 \\

& Ast-Grep & 305 & 45.4 & \textbf{140} & \textbf{97} & \textbf{82.6} & 187 & 404 & 27.7 & 336 \\

& GritQL & 2 & 99.6 & 212 & \textbf{0} & \textbf{100.0} & 248 & 1 & 99.8 & \textbf{185} \\
\midrule
\multicolumn{11}{l}{\textbf{API Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=605)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & \textbf{54} & \textbf{91.1} & 293 & 63 & 89.6 & 394 & 367 & 39.3 & \textbf{183} \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{39} & \textbf{93.6} & \textbf{241} & 89 & 85.3 & 323 & 190 & 68.6 & 768 \\

& Ast-Grep & 310 & 48.8 & \textbf{183} & \textbf{113} & \textbf{81.3} & 349 & 462 & 23.6 & 399 \\

& GritQL & 3 & 99.5 & 365 & \textbf{0} & \textbf{100.0} & 471 & 3 & 99.5 & \textbf{255} \\
\midrule
\multicolumn{11}{l}{\textbf{Language Version Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45)\end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & \textbf{0} & \textbf{100.0} & 113 & \textbf{0} & \textbf{100.0} & 141 & 20 & 55.6 & \textbf{112} \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{0} & \textbf{100.0} & \textbf{113} & 1 & 97.8 & 146 & 6 & 86.7 & 173 \\

& Ast-Grep & 19 & 57.8 & \textbf{119} & \textbf{12} & \textbf{73.3} & 165 & 32 & 28.9 & 198 \\

& GritQL & \textbf{0} & \textbf{100.0} & \textbf{139} & \textbf{0} & \textbf{100.0} & 161 & 1 & \textbf{100.0} & 161 \\


\bottomrule
\end{tabular*}
\caption*{\textit{Metrics: F = Failures; RA = Rule Applicability rate; NT = Number of Generated Tokens; Bold = top 1\% of results for each tool.}}
\end{table}

==> tables/tab-results-rq1bis.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Soundness of Generated Transformation Rules per Dataset, Tool, and LLM (Grouped by Scenario)}
\vspace{-1em}
\label{tab:results-rq1-bis}
\begin{tabular}{l *{3}{r@{\hspace{6pt}}r@{\hspace{6pt}}r}}
\toprule
\textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& \textbf{F} & \textbf{RA} & \textbf{NT}
& \textbf{F} & \textbf{RA} & \textbf{NT}
& \textbf{F} & \textbf{RA} & \textbf{NT} \\ % Fixed header
\midrule

\multicolumn{10}{c}{\textbf{API Misuse}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{Galappaththi et al. (n=43)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 3 & 93\% & 192 & \textbf{2} & \textbf{95.3\%} & 208 & 18 & 58.1\% & \textbf{166} \\
Comby \textit{(no RAG)} & \textbf{0} & \textbf{100\%} & \textbf{185} & \textbf{0} & \textbf{100\%} & 202 & 8 & 81.4\% & 264 \\
Ast-Grep & 17 & 60.5\% & \textbf{170} & \textbf{3} & \textbf{93\%} & 228 & 25 & 40.5\% & 342 \\
GritQL & 2 & 95.3\% & 253 & \textbf{0} & \textbf{100\%} & \textbf{215} & 1 & 97.7\% & 293 \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Program Repair}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{ManySStuBs4J (n=528)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 9 & 98.9\% & \textbf{90} & \textbf{5} & \textbf{99.2\%} & 225 & 335 & 36.6\% & 212 \\
Comby \textit{(no RAG)} & \textbf{12} & \textbf{97.9\%} & \textbf{88} & 88 & 83.5\% & 171 & 128 & 76.1\% & 995 \\
Ast-Grep & 219 & 58.7\% & 108 & \textbf{77} & \textbf{85.6\%} & \textbf{108} & 448 & 15.5\% & 557 \\
GritQL & 5 & 99.4\% & \textbf{148} & 5 & 99.4\% & 221 & \textbf{4} & \textbf{99.8\%} & 242 \\

\addlinespace[3pt]
\multicolumn{10}{c}{\emph{Defects4J (n=427)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 34 & 92.3\% & 160 & \textbf{4} & \textbf{99.1\%} & 211 & 264 & 38\% & \textbf{124} \\
Comby \textit{(no RAG)} & \textbf{24} & \textbf{94.8\%} & \textbf{134} & 89 & 79.1\% & 173 & 125 & 71.1\% & 239 \\
Ast-Grep & 203 & 53.8\% & 152 & \textbf{92} & \textbf{78.4\%} & 179 & 302 & 29.1\% & \textbf{197} \\
GritQL & 6 & 98.6\% & 201 & \textbf{0} & \textbf{100\%} & 240 & \textbf{0} & \textbf{100\%} & \textbf{174} \\

\addlinespace[3pt]
\multicolumn{10}{c}{\emph{BugsInPy (n=559)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 36 & 93.6\% & \textbf{158} & \textbf{34} & \textbf{93.9\%} & 213 & 429 & 23.3\% & 159 \\
Comby \textit{(no RAG)} & \textbf{18} & \textbf{96.8\%} & \textbf{149} & 178 & 68.2\% & 169 & 134 & 76\% & 201 \\
Ast-Grep & 305 & 45.4\% & \textbf{140} & \textbf{97} & \textbf{82.6\%} & 187 & 404 & 27.7\% & 336 \\
GritQL & 2 & 99.6\% & 212 & \textbf{0} & \textbf{100\%} & 248 & 1 & 99.8\% & \textbf{185} \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{API Migration}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{PyMigBench (n=605)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & \textbf{54} & \textbf{91.1\%} & 293 & 63 & 89.6\% & 394 & 367 & 39.3\% & \textbf{183} \\
Comby \textit{(no RAG)} & \textbf{39} & \textbf{93.6\%} & \textbf{241} & 89 & 85.3\% & 323 & 190 & 68.6\% & 768 \\
Ast-Grep & 310 & 48.8\% & \textbf{183} & \textbf{113} & \textbf{81.3\%} & 349 & 462 & 23.6\% & 399 \\
GritQL & 3 & 99.5\% & 365 & \textbf{0} & \textbf{100\%} & 471 & 3 & 99.5\% & \textbf{255} \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Language Version Migration}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{JMigBench (n=45)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & \textbf{0} & \textbf{100\%} & 113 & \textbf{0} & \textbf{100\%} & 141 & 20 & 55.6\% & \textbf{112} \\
Comby \textit{(no RAG)} & \textbf{0} & \textbf{100\%} & \textbf{113} & 1 & 97.8\% & 146 & 6 & 86.7\% & 173 \\
Ast-Grep & 19 & 57.8\% & \textbf{119} & \textbf{12} & \textbf{73.3\%} & 165 & 32 & 28.9\% & 198 \\
GritQL & \textbf{0} & \textbf{100\%} & \textbf{139} & \textbf{0} & \textbf{100\%} & 161 & 1 & \textbf{100\%} & 161 \\
\bottomrule
\end{tabular}
\newline\textbf{\textit{F: Failures; RA: Rule Applicability rate; NT: Number of Generated Tokens}}
\vspace{\vspacesarebad} % à modifier dans main.tex pour être consistant
\end{table}

==> tables/tab-results-rq2-datasets-agg.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per DSL and LLM}
\label{tab:results-rq2-datasets-agg}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{DSL}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%} \\

\midrule

\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
Mean over DSLs & 3.2 & 55.1 & 9 & 2.3 & 105.7 & 10 & 5.0 & 45.3 & 8 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
Mean over DSLs & 2.0 & 69.2 & 16 & 1.8 & 123.0 & 9 & 7.1 & 42.4 & 4 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
Mean over DSLs & 4.2 & 67.1 & 9 & 3.9 & 154.6 & 5 & 10.6 & 41.7 & 2 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
Mean over DSLs & 1.7 & 115.2 & 17 & 1.6 & 210.1 & 14 & 4.1 & 47.0 & 7 \\

\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: NR = Number of Rules, SR = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq2-datasets.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per Scenario, Tool, and LLM}
\label{tab:results-rq2-datasets}
\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l l ccc ccc ccc @{}}
\toprule
\textbf{Scenario} & \textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
& 
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%} \\

\midrule

\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
& Comby & 3.4 & 57.3 & 7 & 1.6 & 162.8 & 10 & 3.9 & 44.5 & 14 \\
& Comby (no RAG) & 3.4 & 53.9 & 7 & 2.1 & 115.3 & 6 & 7.3 & 41.4 & 3 \\
& Ast-Grep & 3.1 & 39.6 & 17 & 3.6 & 51.0 & 9 & 4.3 & 48.3 & 15 \\
& GritQL & 2.8 & 69.6 & 7 & 1.9 & 93.8 & 13 & 4.2 & 46.9 & 0 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
& Comby & 1.9 & 80.2 & 15 & 1.7 & 179.2 & 7 & 4.8 & 45.5 & 4 \\
& Comby (no RAG) & 1.9 & 69.0 & 16 & 1.7 & 127.1 & 4 & 14.9 & 38.1 & 7 \\
& Ast-Grep & 2.1 & 53.8 & 19 & 2.1 & 71.1 & 14 & 5.9 & 37.4 & 5 \\
& GritQL & 2.0 & 74.1 & 14 & 1.7 & 114.4 & 12 & 2.9 & 48.6 & 1 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
& Comby & 4.7 & 90.4 & 7 & 3.0 & 242.1 & 3 & 5.9 & 39.6 & 4 \\
& Comby (no RAG) & 4.6 & 68.8 & 9 & 3.6 & 160.4 & 3 & 24.5 & 35.4 & 1 \\
& Ast-Grep & 3.3 & 36.3 & 14 & 5.4 & 70.2 & 8 & 8.0 & 52.5 & 4 \\
& GritQL & 4.4 & 73.0 & 7 & 3.7 & 145.5 & 7 & 4.1 & 39.1 & 0 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
& Comby & 1.8 & 115.8 & 17 & 1.1 & 278.6 & 13 & 3.2 & 45.8 & 10 \\
& Comby (no RAG) & 1.6 & 135.1 & 14 & 1.1 & 285.1 & 7 & 5.7 & 41.9 & 7 \\
& Ast-Grep & 2.0 & 60.0 & 20 & 2.9 & 72.1 & 22 & 4.7 & 47.2 & 11 \\
& GritQL & 1.3 & 149.8 & 16 & 1.2 & 204.7 & 13 & 2.6 & 53.2 & 0 \\

\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: NR = Number of Rules, SR = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq2-dsl.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per DSL and LLM}
\label{tab:results-rq2-dsl}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{DSL}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%} \\

\midrule

Comby & 2.6 & 84.0 & 13 & 1.8 & 203.5 & 8 & 4.6 & 44.4 & 7 \\
Comby (no RAG) & 2.6 & 77.4 & 13 & 2.0 & 157.0 & 5 & 13.7 & 38.8 & 5 \\
Ast-Grep & 2.4 & 49.6 & 18 & 3.0 & 67.8 & 14 & 5.8 & 43.4 & 7 \\
GritQL & 2.4 & 85.8 & 12 & 2.0 & 131.2 & 12 & 3.3 & 47.5 & 0 \\


\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: NR = Number of Rules, SR = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq2-tools.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per Dataset and LLM}
\label{tab:results-rq2-tools}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{Benchmarks}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
& \textbf{NR} & \textbf{SR} & \textbf{MTR\%} \\
\midrule

\multicolumn{10}{l}{\textbf{API Misuse}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} Galappaththi et al. \\ \footnotesize (n=43) \end{tabular}
& 3.2 & 55.1 & 9
& 2.3 & 105.7 & 10
& 5.0 & 45.3 & 8 \\

\midrule
\multicolumn{10}{l}{\textbf{Program Repair}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528) \end{tabular}
& 1.9 & 62.0 & 17
& 1.7 & 94.9 & 13
& 12.5 & 52.0 & 7 \\

\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427) \end{tabular}
& 1.9 & 73.5 & 16
& 1.7 & 138.6 & 9
& 4.0 & 30.3 & 1 \\

\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=493) \end{tabular}
& 2.1 & 72.3 & 15
& 1.9 & 135.4 & 7
& 4.9 & 45.0 & 4 \\

\midrule
\multicolumn{10}{l}{\textbf{API Migration}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=661) \end{tabular}
& 4.2 & 67.1 & 9
& 3.9 & 154.6 & 5
& 10.6 & 41.7 & 2 \\

\midrule
\multicolumn{10}{l}{\textbf{Language Version Migration}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45) \end{tabular}
& 1.7 & 115.2 & 17
& 1.6 & 210.1 & 14
& 4.1 & 47.0 & 7 \\

\bottomrule
\end{tabular*}
\caption*{\textit{Metrics: NR = Number of Rules, SR = Size of Rules, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq2.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Structural Completeness of Generated Rules per Dataset, Tool, and LLM (Grouped by Scenario)}
\label{tab:results-rq2}
\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l l *{3}{c c c} @{}}
\toprule
\textbf{Benchmarks} & \textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
& & \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
  & \textbf{NR} & \textbf{SR} & \textbf{MTR\%}
  & \textbf{NR} & \textbf{SR} & \textbf{MTR\%} \\
\midrule

\multicolumn{11}{l}{\textbf{API Misuse}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Galappaththi \\ et al. \\ \footnotesize (n=43) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 3.4 & 57.3 & 7\% & 1.6 & 162.8 & 10\% & 3.9 & 44.5 & 14\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 3.4 & 53.9 & 7\% & 2.1 & 115.3 & 6\% & 7.3 & 41.4 & 3\% \\

& Ast-Grep & 3.1 & 39.6 & 17\% & 3.6 & 51.0 & 9\% & 4.3 & 48.3 & 15\% \\

& GritQL & 2.8 & 69.6 & 7\% & 1.9 & 93.8 & 13\% & 4.2 & 46.9 & 0\% \\
\midrule
\multicolumn{11}{l}{\textbf{Program Repair}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 1.8 & 63.4 & 18\% & 1.6 & 167.6 & 10\% & 6.1 & 48.9 & 4\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 1.9 & 63.5 & 17\% & 1.9 & 73.8 & 6\% & 0.0 & 0.0 & 0\% \\

& Ast-Grep & 2.0 & 55.1 & 20\% & 1.8 & 58.6 & 19\% & 11.6 & 61.2 & 6\% \\

& GritQL & 1.9 & 65.9 & 14\% & 1.6 & 79.5 & 16\% & 3.5 & 54.3 & 1\% \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 1.8 & 96.2 & 13\% & 1.6 & 183.8 & 7\% & 3.9 & 45.2 & 4\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 1.9 & 67.5 & 16\% & 1.6 & 160.1 & 3\% & 9.5 & 27.1 & 1\% \\

& Ast-Grep & 2.1 & 51.6 & 19\% & 2.0 & 78.1 & 14\% & 0.0 & 0.0 & 0\% \\

& GritQL & 1.9 & 78.5 & 15\% & 1.7 & 132.6 & 11\% & 2.4 & 48.7 & 0\% \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=493) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 2.1 & 80.8 & 15\% & 1.7 & 186.2 & 4\% & 4.4 & 42.4 & 6\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 2.1 & 75.9 & 13\% & 1.7 & 147.4 & 3\% & 5.8 & 43.6 & 2\% \\

& Ast-Grep & 2.0 & 54.8 & 18\% & 2.3 & 76.7 & 11\% & 6.7 & 51.3 & 8\% \\

& GritQL & 2.1 & 77.8 & 13\% & 1.9 & 131.3 & 8\% & 2.8 & 42.7 & 1\% \\
\midrule
\multicolumn{11}{l}{\textbf{API Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=661) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 4.7 & 90.4 & 7\% & 3.0 & 242.1 & 3\% & 5.9 & 39.6 & 4\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 4.6 & 68.8 & 9\% & 3.6 & 160.4 & 3\% & 24.5 & 35.4 & 1\% \\

& Ast-Grep & 3.3 & 36.3 & 14\% & 5.4 & 70.2 & 8\% & 8.0 & 52.5 & 4\% \\

& GritQL & 4.4 & 73.0 & 7\% & 3.7 & 145.5 & 7\% & 4.1 & 39.1 & 0\% \\
\midrule
\multicolumn{11}{l}{\textbf{Language Version Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 1.8 & 115.8 & 17\% & 1.1 & 278.6 & 13\% & 3.2 & 45.8 & 10\% \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 1.6 & 135.1 & 14\% & 1.1 & 285.1 & 7\% & 5.7 & 41.9 & 7\% \\

& Ast-Grep & 2.0 & 60.0 & 20\% & 2.9 & 72.1 & 22\% & 4.7 & 47.2 & 11\% \\

& GritQL & 1.3 & 149.8 & 16\% & 1.2 & 204.7 & 13\% & 2.6 & 53.2 & 0\% \\

\bottomrule
\end{tabular*}
\caption*{\textit{Metrics: NR = Number of rules; SR = Size of Rules; MTR = Metavariables Token Ratio}}
\end{table}

==> tables/tab-results-rq2bis.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Structural Completeness of Generated Rules per Dataset, Tool, and LLM (Grouped by Scenario)}
\vspace{-1em}
\label{tab:results-rq2-bis}
\begin{tabular*}{\linewidth}{l *{3}{r@{\hspace{6pt}}r@{\hspace{5pt}}r}}
\toprule
\textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& \textbf{NR} & \textbf{SR} & \textbf{MTR}
& \textbf{NR} & \textbf{SR} & \textbf{MTR}
& \textbf{NR} & \textbf{SR} & \textbf{MTR} \\
\midrule

\multicolumn{10}{c}{\textbf{API Misuse}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{Galappaththi et al. (n=43)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 3.4 & 57.3 & 7\% & 1.6 & 162.8 & 10\% & 3.9 & 44.5 & 14\% \\
Comby \textit{(no RAG)} & 3.4 & 53.9 & 7\% & 2.1 & 115.3 & 6\% & 7.3 & 41.4 & 3\% \\
Ast-Grep & 3.1 & 39.6 & 17\% & 3.6 & 51.0 & 9\% & 4.3 & 48.3 & 15\% \\
GritQL & 2.8 & 69.6 & 7\% & 1.9 & 93.8 & 13\% & 4.2 & 46.9 & 0\% \\
\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Program Repair}} \\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{ManySStuBs4J (n=528)}} \\
\addlinespace[1pt]
Comby \textit{(RAG)} & 1.8 & 63.4 & 18\% & 1.6 & 167.6 & 10\% & 6.1 & 48.9 & 4\% \\
Comby \textit{(no RAG)} & 1.9 & 63.5 & 17\% & 1.9 & 73.8 & 6\% & 0.0 & 0.0 & 0\% \\
Ast-Grep & 2.0 & 55.1 & 20\% & 1.8 & 58.6 & 19\% & 11.6 & 61.2 & 6\% \\
GritQL & 1.9 & 65.9 & 14\% & 1.6 & 79.5 & 16\% & 3.5 & 54.3 & 1\% \\
\addlinespace[3pt]
\multicolumn{10}{c}{\emph{Defects4J (n=427)}} \\
\addlinespace[1pt]
Comby \textit{(RAG)} & 1.8 & 96.2 & 13\% & 1.6 & 183.8 & 7\% & 3.9 & 45.2 & 4\% \\
Comby \textit{(no RAG)} & 1.9 & 67.5 & 16\% & 1.6 & 160.1 & 3\% & 9.5 & 27.1 & 1\% \\
Ast-Grep & 2.1 & 51.6 & 19\% & 2.0 & 78.1 & 14\% & 4.2 & 31.5 & 0\% \\
GritQL & 1.9 & 78.5 & 15\% & 1.7 & 132.6 & 11\% & 2.4 & 48.7 & 0\% \\
\addlinespace[3pt]
\multicolumn{10}{c}{\emph{BugsInPy (n=559)}} \\
\addlinespace[1pt]
Comby \textit{(RAG)} & 2.1 & 80.8 & 15\% & 1.7 & 186.2 & 4\% & 4.4 & 42.4 & 6\% \\
Comby \textit{(no RAG)} & 2.1 & 75.9 & 13\% & 1.7 & 147.4 & 3\% & 5.8 & 43.6 & 2\% \\
Ast-Grep & 2.0 & 54.8 & 18\% & 2.3 & 76.7 & 11\% & 6.7 & 51.3 & 8\% \\
GritQL & 2.1 & 77.8 & 13\% & 1.9 & 131.3 & 8\% & 2.8 & 42.7 & 1\% \\
\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{API Migration}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{PyMigBench (n=605)}} \\
\addlinespace[1pt]
Comby \textit{(RAG)} & 4.7 & 90.4 & 7\% & 3.0 & 242.1 & 3\% & 5.9 & 39.6 & 4\% \\
Comby \textit{(no RAG)} & 4.6 & 68.8 & 9\% & 3.6 & 160.4 & 3\% & 24.5 & 35.4 & 1\% \\
Ast-Grep & 3.3 & 36.3 & 14\% & 5.4 & 70.2 & 8\% & 8.0 & 52.5 & 4\% \\
GritQL & 4.4 & 73.0 & 7\% & 3.7 & 145.5 & 7\% & 4.1 & 39.1 & 0\% \\
\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Language Version Migration}} \\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{JMigBench (n=45)}} \\
\addlinespace[1pt]
Comby \textit{(RAG)} & 1.8 & 115.8 & 17\% & 1.1 & 278.6 & 13\% & 3.2 & 45.8 & 10\% \\
Comby \textit{(no RAG)} & 1.6 & 135.1 & 14\% & 1.1 & 285.1 & 7\% & 5.7 & 41.9 & 7\% \\
Ast-Grep & 2.0 & 60.0 & 20\% & 2.9 & 72.1 & 22\% & 4.7 & 47.2 & 11\% \\
GritQL & 1.3 & 149.8 & 16\% & 1.2 & 204.7 & 13\% & 2.6 & 53.2 & 0\% \\
\bottomrule
\end{tabular*}
\newline\textbf{\textit{NR: Number of rules; SR: Size of Rules; MTR: Metavariables Token Ratio}}
\vspace{\vspacesarebad} % à modifier dans main.tex pour être consistant
\end{table}

==> tables/tab-results-rq3-datasets-agg.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per DSL and LLM}
\label{tab:results-rq3-datasets-agg}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{DSL}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM} \\

\midrule

\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
Mean over DSLs & 83.6 & 58.3 & 58.3 & 86.7 & 56.6 & 56.6 & 78.4 & 22.8 & 22.8 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
Mean over DSLs & 88.1 & 32.4 & 41.0 & 89.6 & 42.9 & 50.1 & 83.3 & 9.8 & 18.2 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
Mean over DSLs & 75.3 & 41.6 & 41.6 & 77.1 & 48.2 & 48.2 & 70.7 & 15.8 & 15.8 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
Mean over DSLs & 84.6 & 46.0 & 46.6 & 83.2 & 45.4 & 47.4 & 64.1 & 11.9 & 15.1 \\

\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: TD = Number of Rules, EM = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq3-datasets.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per Scenario, Tool, and LLM}
\label{tab:results-rq3-datasets}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l l ccc ccc ccc @{}}
\toprule
\textbf{Scenario} & \textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
& 
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM} \\

\midrule

\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Misuse} \\ \footnotesize (n=43)\end{tabular}} \\
\midrule
& Comby & 82.8 & 67.5 & 67.5 & 88.1 & 63.4 & 63.4 & 80.1 & 24.0 & 24.0 \\
& Comby (no RAG) & 79.7 & 53.5 & 53.5 & 82.1 & 48.8 & 48.8 & 72.9 & 25.7 & 25.7 \\
& Ast-Grep & 85.6 & 53.8 & 53.8 & 88.6 & 67.5 & 67.5 & 83.1 & 17.6 & 17.6 \\
& GritQL & 86.3 & 58.5 & 58.5 & 88.1 & 46.5 & 46.5 & 77.6 & 23.8 & 23.8 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Program Repair} \\ \footnotesize (n=1514)\end{tabular}} \\
\midrule
& Comby & 87.8 & 33.0 & 41.6 & 82.0 & 34.3 & 40.6 & 79.9 & 9.0 & 15.7 \\
& Comby (no RAG) & 84.7 & 31.0 & 39.9 & 88.7 & 40.1 & 46.4 & 84.1 & 12.4 & 24.2 \\
& Ast-Grep & 88.3 & 41.6 & 49.9 & 92.6 & 55.3 & 64.0 & 79.0 & 9.9 & 11.9 \\
& GritQL & 91.5 & 23.8 & 32.7 & 94.9 & 41.8 & 49.1 & 90.2 & 7.9 & 21.1 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{API Migration} \\ \footnotesize (n=605)\end{tabular}} \\
\midrule
& Comby & 69.1 & 43.2 & 43.2 & 69.4 & 45.6 & 45.6 & 67.6 & 12.2 & 12.2 \\
& Comby (no RAG) & 65.9 & 41.7 & 41.7 & 69.4 & 49.8 & 49.8 & 72.1 & 25.5 & 25.5 \\
& Ast-Grep & 88.0 & 46.1 & 46.1 & 89.1 & 57.5 & 57.5 & 66.9 & 8.4 & 8.4 \\
& GritQL & 78.0 & 35.2 & 35.2 & 80.6 & 40.0 & 40.0 & 76.0 & 17.3 & 17.3 \\
\midrule
\multicolumn{10}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Language Version Migration} \\ \footnotesize (n=45)\end{tabular}} \\
\midrule
& Comby & 91.0 & 68.9 & 68.9 & 87.0 & 60.0 & 60.0 & 67.8 & 20.0 & 28.0 \\
& Comby (no RAG) & 88.8 & 62.2 & 64.4 & 81.0 & 45.5 & 45.5 & 58.0 & 23.1 & 25.6 \\
& Ast-Grep & 81.6 & 30.8 & 30.8 & 87.7 & 51.5 & 57.6 & 55.7 & 0.0 & 0.0 \\
& GritQL & 76.9 & 22.2 & 22.2 & 76.9 & 24.4 & 26.7 & 74.8 & 4.5 & 6.8 \\

\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: NR = Number of Rules, SR = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq3-dsl.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Characteristics of Generated Transformation Rules per DSL and LLM}
\label{tab:results-rq3-dsl}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{DSL}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM} \\

\midrule

Comby & 84.4 & 46.4 & 50.7 & 81.8 & 45.3 & 48.5 & 75.9 & 13.8 & 18.5 \\
Comby (no RAG) & 81.4 & 41.7 & 46.5 & 83.1 & 44.1 & 47.2 & 75.9 & 18.6 & 24.9 \\
Ast-Grep & 86.7 & 42.6 & 46.7 & 90.6 & 57.1 & 62.5 & 73.8 & 9.3 & 10.3 \\
GritQL & 86.0 & 31.2 & 35.7 & 88.4 & 39.4 & 43.4 & 83.2 & 11.5 & 18.6 \\

\bottomrule
\end{tabular*}

\caption*{\textit{Metrics: TD = Number of Rules, EM = Rule Size, MTR = Match Rate}}
\end{table}

==> tables/tab-results-rq3-tools.tex <==
\begin{table}[H]
\centering
\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Syntactic and Semantic Alignment of Generated Transformations per Dataset and LLM (Averaged Across DSLs)}
\label{tab:results-rq3-tools}
\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
\textbf{Benchmarks}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT-5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM} \\
\midrule

\multicolumn{10}{l}{\textbf{API Misuse}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} Galappaththi et al. \\ \footnotesize (n=43) \end{tabular} & 83.6 & 58.3 & 58.3 & 86.7 & 56.6 & 56.6 & 78.4 & 22.8 & 22.8 \\
\midrule
\multicolumn{10}{l}{\textbf{Program Repair}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528) \end{tabular} & 95.8 & 47.3 & 69.3 & 96.8 & 58.2 & 76.4 & 83.9 & 14.8 & 37.0 \\
\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427) \end{tabular} & 90.9 & 27.1 & 31.0 & 92.9 & 38.4 & 41.7 & 89.8 & 6.4 & 9.7 \\
\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=493) \end{tabular} & 77.6 & 22.7 & 22.7 & 79.0 & 32.1 & 32.1 & 76.2 & 8.1 & 8.1 \\
\midrule
\multicolumn{10}{l}{\textbf{API Migration}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=661) \end{tabular} & 75.3 & 41.6 & 41.6 & 77.1 & 48.2 & 48.2 & 70.7 & 15.8 & 15.8 \\
\midrule
\multicolumn{10}{l}{\textbf{Language Version Migration}} \\
\midrule
\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45) \end{tabular} & 84.6 & 46.0 & 46.6 & 83.2 & 45.4 & 47.4 & 64.1 & 11.9 & 15.1 \\


\bottomrule
\end{tabular*}
\caption*{\textit{Metrics: TD = Tree Distance rate; EM = Exact Match rate; AM = AST Match rate}}
\end{table}

==> tables/tab-results-rq3.tex <==
\begin{table}[t]
\centering

\setlength{\tabcolsep}{3pt}
\footnotesize
\caption{Syntactic and Semantic Alignment of Generated Transformations per Dataset, Tool, and LLM (Grouped by Scenario)}
\label{tab:results-rq3}
\hspace*{-0.5cm} % to shift the table on the left
\begin{tabular}{l l *{3}{c c c}}
\toprule
\textbf{Benchmarks} & \textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
& & \textbf{TD} & \textbf{EM} & \textbf{AM}
  & \textbf{TD} & \textbf{EM} & \textbf{AM}
  & \textbf{TD} & \textbf{EM} & \textbf{AM} \\
\midrule

\multicolumn{11}{l}{\textbf{API Misuse}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Galappaththi \\ et al. \\ \footnotesize (n=43) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 82.8 & \textbf{67.5} & \textbf{67.5} & \textbf{88.1} & 63.4 & 63.4 & 80.1 & 24.0 & 24.0 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 79.7 & \textbf{53.5} & \textbf{53.5} & \textbf{82.1} & 48.8 & 48.8 & 72.9 & 25.7 & 25.7 \\

& Ast-Grep & 85.6 & 53.8 & 53.8 & \textbf{88.6} & \textbf{67.5} & \textbf{67.5} & 83.1 & 17.6 & 17.6 \\

& GritQL & 86.3 & \textbf{58.5} & \textbf{58.5} & \textbf{88.1} & 46.5 & 46.5 & 77.6 & 23.8 & 23.8 \\
\midrule
\multicolumn{11}{l}{\textbf{Program Repair}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} ManySStuBs4J \\ \footnotesize (n=528) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & \textbf{96.7} & 45.1 & 69.2 & \textbf{97.0} & \textbf{57.6} & \textbf{74.8} & 83.6 & 11.9 & 29.5 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{97.3} & 45.7 & 68.2 & \textbf{97.7} & \textbf{56.4} & \textbf{72.7} & 89.5 & 18.2 & 47.8 \\

& Ast-Grep & 90.8 & 52.1 & 71.5 & \textbf{94.3} & \textbf{62.5} & \textbf{82.0} & 68.6 & 23.8 & 30.0 \\

& GritQL & \textbf{98.5} & 46.1 & 68.5 & \textbf{98.1} & \textbf{56.4} & \textbf{76.1} & 93.9 & 5.3 & 40.6 \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Defects4J \\ \footnotesize (n=427) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 92.5 & 31.6 & 33.2 & \textbf{94.1} & \textbf{33.6} & \textbf{35.3} & 84.3 & 8.0 & 10.5 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 89.4 & 28.1 & 32.3 & \textbf{94.0} & \textbf{35.0} & \textbf{37.7} & 84.0 & 9.3 & 15.3 \\

& Ast-Grep & \textbf{89.5} & 41.3 & 46.6 & \textbf{90.0} & \textbf{49.4} & \textbf{56.0} & 70.5 & 5.2 & 8.4 \\

& GritQL & 92.2 & 7.4 & 11.7 & \textbf{93.6} & \textbf{35.4} & \textbf{37.8} & 90.7 & 8.5 & 12.9 \\
\addlinespace
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} BugsInPy \\ \footnotesize (n=493) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & \textbf{74.3} & \textbf{22.4} & \textbf{22.4} & 54.9 & 11.8 & 11.8 & 71.8 & 6.9 & 6.9 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 67.3 & 19.0 & 19.0 & 74.5 & \textbf{28.9} & \textbf{28.9} & \textbf{78.6} & 9.6 & 9.6 \\

& Ast-Grep & 84.7 & 31.5 & 31.5 & \textbf{93.7} & \textbf{54.1} & \textbf{54.1} & 68.3 & 5.8 & 5.8 \\

& GritQL & 84.0 & 18.0 & 18.0 & \textbf{92.9} & \textbf{33.5} & \textbf{33.5} & 86.0 & 9.9 & 9.9 \\
\midrule
\multicolumn{11}{l}{\textbf{API Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} PyMigBench \\ \footnotesize (n=661) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & 69.1 & 43.2 & 43.2 & \textbf{69.4} & \textbf{45.6} & \textbf{45.6} & 67.6 & 12.2 & 12.2 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & 65.9 & 41.7 & 41.7 & 69.4 & \textbf{49.8} & \textbf{49.8} & \textbf{72.1} & 25.5 & 25.5 \\

& Ast-Grep & 88.0 & 46.1 & 46.1 & \textbf{89.1} & \textbf{57.5} & \textbf{57.5} & 66.9 & 8.4 & 8.4 \\

& GritQL & 78.0 & 35.2 & 35.2 & \textbf{80.6} & \textbf{40.0} & \textbf{40.0} & 76.0 & 17.3 & 17.3 \\
\midrule
\multicolumn{11}{l}{\textbf{Language Version Migration}} \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} JMigBench \\ \footnotesize (n=45) \end{tabular}}
& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(RAG)} \end{tabular} & \textbf{91.0} & \textbf{68.9} & \textbf{68.9} & 87.0 & 60.0 & 60.0 & 67.8 & 20.0 & 28.0 \\

& \begin{tabular}[c]{@{}l@{}} Comby \\ \scriptsize\textit{(no RAG)} \end{tabular} & \textbf{88.8} & \textbf{62.2} & \textbf{64.4} & 81.0 & 45.5 & 45.5 & 58.0 & 23.1 & 25.6 \\

& Ast-Grep & 81.6 & 30.8 & 30.8 & \textbf{87.7} & \textbf{51.5} & \textbf{57.6} & 55.7 & 0.0 & 0.0 \\

& GritQL & \textbf{76.9} & 22.2 & 22.2 & \textbf{76.9 }& \textbf{24.4} & \textbf{26.7} & 74.8 & 4.5 & 6.8 \\

\bottomrule
\end{tabular}
\caption*{\textit{Metrics: TD = Tree Distance rate; EM = Exact Match rate; AM = AST Match rate; Bold = top 1\% of results for each tool.}}
\end{table}

==> tables/tab-results-rq3bis.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Syntactic \removed{and Semantic} Alignment of Generated code per Dataset, Tool, and LLM (Grouped by Scenario)}
\vspace{-1em}
\label{tab:results-rq3-bis}
\begin{tabular}{l *{3}{r@{\hspace{6pt}}r@{\hspace{6pt}}r}}
\toprule
\textbf{Tool}
& \multicolumn{3}{c}{\textbf{GPT-oss-120B}}
& \multicolumn{3}{c}{\textbf{GPT5.4}}
& \multicolumn{3}{c}{\textbf{Llama3.1-8B}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM}
& \textbf{TD} & \textbf{EM} & \textbf{AM} \\
\midrule

\multicolumn{10}{c}{\textbf{API Misuse}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{Galappaththi et al. (n=43)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 82.8 & \textbf{67.5} & \textbf{67.5} & \textbf{88.1} & 63.4 & 63.4 & 80.1 & 24.0 & 24.0 \\
Comby \textit{(no RAG)} & 79.7 & \textbf{53.5} & \textbf{53.5} & \textbf{82.1} & 48.8 & 48.8 & 72.9 & 25.7 & 25.7 \\
Ast-Grep & 85.6 & 53.8 & 53.8 & \textbf{88.6} & \textbf{67.5} & \textbf{67.5} & 83.1 & 17.6 & 17.6 \\
GritQL & 86.3 & \textbf{58.5} & \textbf{58.5} & \textbf{88.1} & 46.5 & 46.5 & 77.6 & 23.8 & 23.8 \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Program Repair}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{ManySStuBs4J (n=528)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & \textbf{96.7} & 45.1 & 69.2 & \textbf{97.0} & \textbf{57.6} & \textbf{74.8} & 83.6 & 11.9 & 29.5 \\
Comby \textit{(no RAG)} & \textbf{97.3} & 45.7 & 68.2 & \textbf{97.7} & \textbf{56.4} & \textbf{72.7} & 89.5 & 18.2 & 47.8 \\
Ast-Grep & 90.8 & 52.1 & 71.5 & \textbf{94.3} & \textbf{62.5} & \textbf{82.0} & 68.6 & 23.8 & 30.0 \\
GritQL & \textbf{98.5} & 46.1 & 68.5 & \textbf{98.1} & \textbf{56.4} & \textbf{76.1} & 93.9 & 5.3 & 40.6 \\

\addlinespace[3pt]
\multicolumn{10}{c}{\emph{Defects4J (n=427)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 92.5 & 31.6 & 33.2 & \textbf{94.1} & \textbf{33.6} & \textbf{35.3} & 84.3 & 8.0 & 10.5 \\
Comby \textit{(no RAG)} & 89.4 & 28.1 & 32.3 & \textbf{94.0} & \textbf{35.0} & \textbf{37.7} & 84.0 & 9.3 & 15.3 \\
Ast-Grep & \textbf{89.5} & 41.3 & 46.6 & \textbf{90.0} & \textbf{49.4} & \textbf{56.0} & 70.5 & 5.2 & 8.4 \\
GritQL & 92.2 & 7.4 & 11.7 & \textbf{93.6} & \textbf{35.4} & \textbf{37.8} & 90.7 & 8.5 & 12.9 \\

\addlinespace[3pt]
\multicolumn{10}{c}{\emph{BugsInPy (n=559)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & \textbf{74.3} & \textbf{22.4} & \textbf{22.4} & 54.9 & 11.8 & 11.8 & 71.8 & 6.9 & 6.9 \\
Comby \textit{(no RAG)} & 67.3 & 19.0 & 19.0 & 74.5 & \textbf{28.9} & \textbf{28.9} & \textbf{78.6} & 9.6 & 9.6 \\
Ast-Grep & 84.7 & 31.5 & 31.5 & \textbf{93.7} & \textbf{54.1} & \textbf{54.1} & 68.3 & 5.8 & 5.8 \\
GritQL & 84.0 & 18.0 & 18.0 & \textbf{92.9} & \textbf{33.5} & \textbf{33.5} & 86.0 & 9.9 & 9.9 \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{API Migration}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{PyMigBench (n=605)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & 69.1 & 43.2 & 43.2 & \textbf{69.4} & \textbf{45.6} & \textbf{45.6} & 67.6 & 12.2 & 12.2 \\
Comby \textit{(no RAG)} & 65.9 & 41.7 & 41.7 & 69.4 & \textbf{49.8} & \textbf{49.8} & \textbf{72.1} & 25.5 & 25.5 \\
Ast-Grep & 88.0 & 46.1 & 46.1 & \textbf{89.1} & \textbf{57.5} & \textbf{57.5} & 66.9 & 8.4 & 8.4 \\
GritQL & 78.0 & 35.2 & 35.2 & \textbf{80.6} & \textbf{40.0} & \textbf{40.0} & 76.0 & 17.3 & 17.3 \\

\cmidrule(lr){1-10}
\multicolumn{10}{c}{\textbf{Language Version Migration}}\\
\addlinespace[1pt]
\multicolumn{10}{c}{\emph{JMigBench (n=45)}}\\
\addlinespace[1pt]
Comby \textit{(RAG)} & \textbf{91.0} & \textbf{68.9} & \textbf{68.9} & 87.0 & 60.0 & 60.0 & 67.8 & 20.0 & 28.0 \\
Comby \textit{(no RAG)} & \textbf{88.8} & \textbf{62.2} & \textbf{64.4} & 81.0 & 45.5 & 45.5 & 58.0 & 23.1 & 25.6 \\
Ast-Grep & 81.6 & 30.8 & 30.8 & \textbf{87.7} & \textbf{51.5} & \textbf{57.6} & 55.7 & 0.0 & 0.0 \\
GritQL & \textbf{76.9} & 22.2 & 22.2 & \textbf{76.9} & \textbf{24.4} & \textbf{26.7} & 74.8 & 4.5 & 6.8 \\
\bottomrule
\end{tabular}
\textbf{\textit{TD: Tree Distance; EM: Exact Match rate; AM: AST Match rate}}
\vspace{\vspacesarebad} % à modifier dans main.tex pour être consistant
\end{table}
